Generative AI for Cel-Animation: A Survey

Traditional Celluloid (Cel) Animation production pipeline encompasses multiple essential steps, including storyboarding, layout design, keyframe animation, inbetweening, and colorization, which demand substantial manual effort, technical expertise, and significant time investment. These challenges have historically impeded the efficiency and scalability of Cel-Animation production. The rise of generative artificial intelligence (GenAI), encompassing large language models, multimodal models, and diffusion models, offers innovative solutions by automating tasks such as inbetween frame generation, colorization, and storyboard creation. This survey explores how GenAI integration is revolutionizing traditional animation workflows by lowering technical barriers, broadening accessibility for a wider range of creators through tools like AniDoc, ToonCrafter, and AniSora, and enabling artists to focus more on creative expression and artistic innovation. Despite its potential, challenges like visual consistency, stylistic coherence, and ethical considerations persist. Additionally, this paper explores future directions and advancements in AI-assisted animation. For further exploration and resources, please visit our GitHub repository: https://github.com/yunlong10/Awesome-AI4Animation

==> tab/dataset.tex <==
\begin{table*}[!ht]
\centering
\caption{This table concisely summarizes cel-animation datasets (Sakuga-42M, AniSora, AnimeRun, ATD-12K, Mixamo-Line240, AnT, PaintBucket-Character) supporting tasks such as comprehension, generation, inbetweening, and colorization. It also lists related datasets (Anim-400K, V2C-Animation, iHarmony4, SSHarmonization, HVIDIT, Alchemist, MangaZero, Ads-1k) relevant to dubbing, harmonization, layout, and scene segmentation. Dataset metrics, including clip and sample counts, clarify their scale and research applicability.}
\label{tab:dataset}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{l| l l l l l l}
\toprule
\textbf{Dataset} & \textbf{Format} & \textbf{Task in Cel}   & \textbf{\#Clips} & \textbf{\#Samples} \\
\midrule
Sakuga-42M~\cite{pan2024sakuga} & Video & Comprehension, Generation  & 1.2M & 42M   \\
AniSora~\cite{jiang2024anisora} & Video & Comprehension, Generation  & 10M &   \\
Anim-400K~\cite{cai2024anim400k} & Video & Dubbing &  & 400K &   \\
V2C-Animation~\cite{chen2022v2c} & Video & Dubbing & 10,217 &  \\
iHarmony4~\cite{cong2020dovenet} & Image & Compositing, Photography (Harmonization) &  & 73,146  \\
SSHarmonization~\cite{jiang2021ssh} & Image & Compositing, Photography (Harmonization)   &  & 216  \\
HVIDIT~\cite{guo2021intrinsic} & Image & Compositing, Photography (Harmonization)   &  & 3,336 \\
Alchemist~\cite{sharma2024alchemist} & Image & Compositing, Photography (T2I Generation)   &  &  \\
AnimeRun~\cite{siyao2022animerun} & Video & Inbetweening, Colorization & 30 & 2,891   \\
ATD-12K~\cite{siyao2021deep} & Image & Inbetweening &  & 12,000 triplets \\
Mixamo-Line240~\cite{siyao2023deep} & Image & Inbetweening &    & 49,262  \\
AnT~\cite{casey2021animation} & Image & Colorization &    & 11,000 \\
PaintBucket-Character~\cite{dai2024learning} & Image & Colorization &    & 14,545 \\
MangaZero~\cite{wu2024diffsensei} & Image & Layout & & 470K \\
Manga109Story~\cite{chen2024manga} & Image & Layout & & 21K \\
Ads-1k~\cite{Tang_2022_ACCV} & Video & Cutting & 1K & \\
% Creative Flow+~\cite{shugrina2019creative} & Image & 3D shape estimation, correspondence, motion &   & 134k  \\
ANITA DATASET~\cite{Anita2024} & Image & Genga, Nigen, Colorization & & 16,000 \\
\bottomrule
\end{tabular}}
\end{table*}

